Algebraic-Dynamical Theory for Quantum Many-body Hamiltonians: A Formalized Approach To Strongly Interacting Systems

Non-commutative algebras and entanglement are two of the most important hallmarks of many-body quantum systems. Dynamical perturbation methods are the most widely used approaches for quantum many-body systems. While study of entanglement-based numerical methods are booming recently, the traditional dynamical perturbation methods have not benefited from study of quantum entanglement. In this work, we formulate an algebraic-dynamical theory (ADT) by combining the power of quantum algebras and dynamical methods in which quantum entanglement naturally emerges as the organizing principle. We start by introducing a complete operator basis set (COBS), with which an arbitrary state, either pure or mixed, can be represented by the expectation values of COBS. Then we establish a complete mapping from a given state to a complete set of dynamical correlation functions of the state through the Heisenberg- and Schwinger-Dyson-equations-of-motion (SDEOM). The completeness of COBS and the mapping ensures ADT to be a mathematically complete framework in principle. Applying ADT to many-body systems on lattices, we find that the quantum entanglement is represented by the cumulant structure of expectation values of the many-body COBS. The cumulant structure of the state forms a hierarchy in correlations. More importantly, such static correlational hierarchy is inherited by the dynamical correlations and their SDEOM. We propose that the dynamical hierarchy is also carried into any perturbative calculation on that state. We demonstrate the validity of such perturbation hierarchy with an explicit example, in which we show that a single-particle-type perturbative calculation fails while a many-body perturbation following the hierarchy succeeds. We also discuss the computation and approximation schemes of ADT and its implications to other strong coupling theories like parton and slave particle methods.

==> adt-sec2.tex <==
\section{From Algebraic Quantum Mechanics to Quantum Dynamics}

In standard quantum mechanics, the first task is to identify a complete set of commuting (with the Hamiltonian $\mH$) observables/operators (CSCO), $\{\hat{A},\hat{B},\hat{C}, \dots\}$, which {\it commute} with the Hamiltonian $\mH$, so that every eigenstates of $\mH$ can be labeled by their eigenvalues $\ket{\epsilon, a,b,c,\dots}$. The time-evolution of observables are described equivalently, either in the Schr\"{o}dinger picture where the state is time-evolved as $\ket{\Psi(t)} = e^{-i t \mH/\hbar} \ket{\Psi(0)}$, or in the Heisenberg picture where the operators are time-evolved as $\hO(t) = e^{-i t \mH/\hbar} ~\hO ~e^{i t \mH/\hbar}$:
\begin{eqnarray}
   \ev{\hO(t)} = \meanvalue{\Psi(t)}{\hO}{\Psi(t)} = \meanvalue{\Psi}{\hO(t)}{\Psi},
\end{eqnarray}
where for $t=0$ the label is omitted.

A conventional way of computing time-dependent correlation functions of an operator $\hO$ is through the so-called moment expansion\cite{recursion-method}:
\begin{eqnarray}
  \label{eq:Ot-recursion}
  \ev{\hO(t)} = \sum_{n=0}^\infty \ev{\hO^{(n)}} \frac{(-i t)^n}{n!},\\
  \begin{split}
  \ev{\hO^{(n)}} &= i^n \left[ \frac{d^n}{dt^n} \ev{\hO(t)} \right]_{t=0} \\
  &= \frac{1}{\hbar^n}\ev{[\dots[[\hO,\mH],\mH],\dots,\mH]},
\end{split}
\end{eqnarray}
where $\hO^{(0)}= \hO$ and the HEOM
\begin{eqnarray}
  \label{eq:HEOM}
 \frac{d}{dt}\hO(t) = - \frac{i}{\hbar}[\hO(t), H] + \left( \frac{\pt \hO}{\pt t} \right)_{\mH}
\end{eqnarray}
is used. If the series of HEOM is cut off for some $n_0$, i.e. $[\hO^{(n_0)}, \mH] = 0$, then $\ev{\hO(t)} $ can be computed exactly. The set of HEOM-generated operators $\{\hO^{(n)}\}$ is termed the Krylov subspace (more commonly, the $\mH$-generated vectors are also referred to as the Krylov subspace). The most important feature of the set $\{\hO^{(n)}\}$ is that it is {\bf algebraically closed} under the action of HEOM.

In many-body theory, the definition need to be extended to multi-point correlation functions\cite{Martin1959}, which is more conveniently done in the Heisenberg picture.
%\begin{widetext}
%\begin{eqnarray}
%  \label{eq:Gn}
%  G_{n}[\hO_1(t_1), \hO_2(t_2), \dots, \hO_{2n}(t_{2n})] =(-i)^{n/2} \meanvalue{\Psi}{ \mT^{\mathcal{P}} \big\{ \hO_1(t_1), \hO_2(t_2), \dots, \hO_n(t_n) \big\} }{\Psi} - \prod_{i=1}^n C^{\mathcal{P}} \ev{\hO_i},
%\end{eqnarray}
%\end{widetext}
%where we generalize the definition and conventions initially introduced by Schwinger in \refdisp{Martin1959a} because we are interested in more general, mostly interacting dominated Hamiltonian systems composed of noncanonical operators.
%
%{\color{blue}** discussion of differences
%
%The superscript $^{\mathcal{P}}$ means a permutational sign structure and $C^{\mathcal{P}}$ is a constant related to the sign structure, both of which remain to be specified later on. The subtraction of the last term removes static correlations. 
%
%*******
Among them, the most important kind of dynamical correlation functions is the two-time correlation functions, which is the main focus of this work. It is also sometimes referred to as the Green's functions. Among various types of the Green's functions, we shall focus on the time-ordered/causal ones defined as
\begin{widetext}
\begin{eqnarray}
  \label{eq:G2-T-order}
  \begin{split}
    & i G[\hO_i(t_i), \hO_f(t_f)]_\pm = \dev{\mT\{ \hO_i(t_i),\hO_f(t_f)\}}_\pm =\ev{\mT \{ \hO_i(t_i) -\ev{\hO_i(t_i)},  \hO_f(t_f) -\ev{\hO_f(t_f)}\} }_\pm\\
    &= \theta(t_i-t_f) \ev{\hO_i(t_i) \hO_f(t_f)} \pm \theta(t_f - t_i) \ev{\hO_f(t_f) \hO_i(t_i)} - (\theta(t_i-t_f) \pm \theta(t_f - t_i)) \ev{\hO_i} \ev{\hO_f}/2,
\end{split}
\end{eqnarray}
\end{widetext}
where $\theta(t)$ is the Heaviside-step-function. Note that for arbitrary operators, we always subtract the static correlations, if any. This is because we solve the $G$'s by taking its time-derivative, so the static correlations are naturally excluded from the solution.

{\color{red} **Note: Although the last line of the above \eqdisp{eq:G2-T-order} is expressed in terms of the inner product of the time-evolved operators as $\ev{\hO_i(t_i) \hO_f(t_f)}$, the expression is {\bf functional} in nature. In some cases, such as in the presence of degenerate energy levels, a direct calculation via computing $\ev{\hO_i(t_i) \hO_f(t_f)}$ would yield a wrong result! (we shall demonstrate that in \refdisp{Ding2021}). The expression with $\theta$-functions must be considered as a complete entity. The mathematically more accurate definition is to define in terms of the Schwinger's source field technique as functional derivatives with respect to the corresponding source fields:
\begin{widetext}
\begin{eqnarray}
  i G[\hO_i(t_i), \hO_f(t_f)]_\pm = -\frac{\delta^2}{\delta \nu_{\hO_i}(t_i) \delta \nu_{\hO_f}(t_f) } \meanvalue{\Psi}{U_{\text{Schw.}}}{\Psi} \Big\vert_{ \nu_{\hO}(t) \rightarrow 0},\\
  U_{\text{Schw.}}= e^{i ~\mT[ \int dt  (\mH + \sum_{\hO} \nu_{\hO}(t) \hO)]}.
\end{eqnarray}
\end{widetext}
Here $U_{\text{Schw.}}$ is the time-evolution operator with (time-dependent) variational sources $\sum_{\hO}\nu_{\hO}(t)  \hO$. The strength of the sources will be taken to zero only at the end of the calculation.
}

These dynamical correlation functions are difficult to compute directly from original definitions, i.e. the time-evolution of the state or the operators, even for simple few-body systems. Instead, the established practice is to apply the HEOM
and convert the HEOM into a set of equations-of-motion for the dynamical correlation functions as
\begin{widetext}
\begin{eqnarray}
  i \hbar \frac{d}{dt_i} G[\hO_i(t_i), \hO_f(t_f)]_\pm = \delta(t_i-t_f) \dev{[\hO_i, \hO_f]_\pm}_\pm + i \dev{\mT\{[\hO_i(t_i), H],\hO_f(t_f)\}}_\pm, 
\end{eqnarray}
\end{widetext}
where 
\begin{eqnarray}
  \dev{[\hO_i, \hO_f]_\pm}_\pm =
  \begin{cases}
    \ev{[\hO_i, \hO_f]},  &\quad \text{for +},\\
    \ev{\{\hO_i, \hO_f\}} - 2 \ev{\hO_i}\ev{\hO_f}, &\quad \text{for -.}
  \end{cases}
\end{eqnarray}
Schwinger-Dyson-equations-of-motion.

In this work, we only discuss time-independent operators and Hamiltonians, the second term of the right hand side of \eqdisp{eq:HEOM} is ignored. By a similar expansion as in \eqdisp{eq:Ot-recursion},
we shall have a series of coupled Schwinger-Dyson-equations-of-motion:
\begin{widetext}
\begin{eqnarray}
  \label{eq:coupled-SDEOM}
  \begin{cases}
  i \frac{d}{dt_i} G[\hO_{i}(t_i), \hO_f(t_f)]_\pm = \delta(t_i-t_f) \ev{[\hO_{i}, \hO_f]_\pm} + G[\hO_{i}^{(1)}(t_i), \hO_f(t_f)]_\pm, \\
  i \frac{d}{dt_i} G[\hO_{i}^{(1)}(t_i), \hO_f(t_f)]_\pm = \delta(t_i-t_f) \ev{[\hO_{i,1}, \hO_f]_\pm} + G[\hO_{i}^{(2)}(t_i), \hO_f(t_f)]_\pm, \\
  \dots  \dots .
\end{cases}
\end{eqnarray}
\end{widetext}
In the above and from here on, we set $\hbar = 1$.
Similarly, if the series of HEOM is cut off at certain level $k$, i.e. $[\hO^{(k)}_{i}(t_i), H] = 0$, \eqdisp{eq:coupled-SDEOM} again become {\bf algebraically closed}. Then, in principle, we can also obtain an exact solution in the frequency space when given all static correlations. \eqdisp{eq:coupled-SDEOM} becomes a set of finite dimensional linear equations of the set of Green's functions $\{ G[\hO^{(n)}_{i}, \hO_f](\omega) \}_{n = 1, 2, 3,\dots, k}$. 

{\color{red} The conjugate correlation functions $\{ G[\hO_{i}, \hO^{(n)}_f](\omega) \}_{n = 1, 2, 3,\dots, k}$ also need to be taken into account. Argument? In order to form a symmetric/Hermitian matrix?} 

The real situation is certainly much more complicated than the above idea. For many-body problems, the generated Krylov-subspace operators $\hO^{(n)}_{i}$s typically are composite operators, meaning they are products or/and superposition of local operators. The complexity of the algebraic relations, as well as the number of $G$s, all grow exponentially with system size.  Next, we propose a systematic way to explore such algebraic-dynamical relations and formulate a new and mathematically rigorous approach for strongly interacting quantum Hamiltonians. 


% LocalWords:  Amongst

